ScaleNet: A Shallow Architecture for Scale Estimation

In this paper, we address the problem of estimating scale factors between images. We formulate the scale estimation problem as a prediction of a probability distribution over scale factors. We design a new architecture, ScaleNet, that exploits dilated convolutions as well as self and cross-correlation layers to predict the scale between images. We demonstrate that rectifying images with estimated scales leads to significant performance improvements for various tasks and methods. Specifically, we show how ScaleNet can be combined with sparse local features and dense correspondence networks to improve camera pose estimation, 3D reconstruction, or dense geometric matching in different benchmarks and datasets. We provide an extensive evaluation on several tasks and analyze the computational overhead of ScaleNet. The code, evaluation protocols, and trained models are publicly available at https://github.com/axelBarroso/ScaleNet.

==> sections/14_notes.tex <==
What is the advantages of Wasserstein metric compared to Kullback-Leibler divergence?:
https://stats.stackexchange.com/questions/295617/what-is-the-advantages-of-wasserstein-metric-compared-to-kullback-leibler-diverg

https://arxiv.org/pdf/1806.02446.pdf : 
Hence, using the UD strategy would induce an over-strengthened loss for the large depth values.
To this end, we propose to perform the discretization using
the SID strategy (as shown in Fig. 4), which uniformed discretizes a given depth interval in log space to down-weight
the training losses in regions with large depth values, so that
our depth estimation network is capable to more accurately
predict relatively small and medium depth and to rationally
estimate large depth values.

Ordinal regression: 

https://github.com/Raschka-research-group/coral-pytorch/blob/main/coral_pytorch/losses.py

https://towardsdatascience.com/how-to-perform-ordinal-regression-classification-in-pytorch-361a2a095a99

https://github.com/dontLoveBugs/DORN_pytorch/blob/master/dorn/models/dorn.py

==> sections/tables/inference_times.tex <==
\begin{table}[]
% \tiny
\footnotesize
\begin{center}
\begin{tabular}{c c c c c c }
\multicolumn{6}{c}{\textbf{Time (ms)}}\\
\hline \noalign{\smallskip}
& DGC-Net & GLU-Net & R2D2 & Key.Net & ScaleNet\\
\hline \noalign{\smallskip}
 & 35.4 & 25.1 & 115 / 384 & 352 / 640 & 33.7 \\
\end{tabular}
\end{center}
\normalsize
\caption{Comparison of computational times in ms for several state-of-the-art methods. We report single and multi-scale times for R2D2 and Key.Net/HardNet. \ab{This may go into supplementary material}}
\label{tab:time_dense}
\end{table}
